CARE: Confounder-Aware Aggregation for Reliable LLM Evaluation

LLM-as-a-judge ensembles are the standard paradigm for scalable evaluation, but their aggregation mechanisms suffer from a fundamental flaw: they implicitly assume that judges provide independent estimates of true quality. However, in practice, LLM judges exhibit correlated errors caused by shared latent confounders -- such as verbosity, stylistic preferences, or training artifacts -- causing standard aggregation rules like majority vote or averaging to provide little gain or even amplify systematic mistakes. To address this, we introduce CARE, a confounder-aware aggregation framework that explicitly models LLM judge scores as arising from both a latent true-quality signal and shared confounding factors. Rather than heuristically re-weighting judges, CARE separates quality from confounders without access to ground-truth labels. We provide theoretical guarantees for identifiability and finite-sample recovery under shared confounders, and we quantify the systematic bias incurred when aggregation models omit confounding latent factors. Across 12 public benchmarks spanning continuous scoring, binary classification, and pairwise preference settings, CARE improves aggregation accuracy, reducing error by up to 26.8\%. Code is released in \href{https://github.com/SprocketLab/CARE}{https://github.com/SprocketLab/CARE}.

==> figures/pgm.tex <==
\usetikzlibrary{positioning}

% pick a nice orange from the Tableau palette
\definecolor{tableauorange}{RGB}{237,125,49}

\tikzset{
  judge/.style={
    circle,
    draw=tableauorange!80!black,
    fill=tableauorange!30,
    minimum size=20pt,
    inner sep=1pt
  },
  quality/.style={
    circle,
    draw=blue!80!black,
    fill=blue!20,
    dashed,
    minimum size=20pt
  },
  confounder/.style={
    circle,
    draw=red!80!black,
    fill=red!20,
    dashed,
    minimum size=20pt
  },
  edgestyle/.style={thick}
}


% \begin{figure*}[t]
  % \centering
  % (a) Only true‐quality
  % \begin{subfigure}[t]{0.32\textwidth}
    % \centering
    % \begin{tikzpicture}[
      % every path/.style=edgestyle
      % ]
      % Judges
      % \node[judge]  (J1a)               {J1};
      % \node[judge, right=1cm of J1a] (J2a)               {J2};
      % \node[judge, right=1cm of J2a] (J3a)            {J3};
      % latent Q
      % \node[quality, above=1cm of J2a] (Q1)                {Q};
      % edges
      % \draw (Q1) -- (J1a);
      % \draw (Q1) -- (J2a);
      % \draw (Q1) -- (J3a);
    % \end{tikzpicture}
    % \caption{Naive: only true‐quality}
  % \end{subfigure}
  % \hfill
  % (b) Connection‐aware
  % \begin{subfigure}[t]{0.32\textwidth}
    % \centering
    % \begin{tikzpicture}[
      % every path/.style=edgestyle
      % ]
      % Judges
      % \node[judge]  (J1b)               {J1};
      % \node[judge, right=1cm of J1b] (J2b)               {J2};
      % \node[judge, right=1cm of J2b] (J3b)            {J3};
      % latent Q
      % \node[quality, above=1cm of J2b] (Q2)                {Q};
      % edges
      % \draw (Q2) -- (J1b);
      % \draw (Q2) -- (J2b);
      % \draw (Q2) -- (J3b);
      % \draw (J2b) -- (J3b);
    % \end{tikzpicture}
    % \caption{Connection-aware}
  % \end{subfigure}
  % \hfill
  % (c) Confounder‐aware
  % \begin{subfigure}[t]{0.32\textwidth}
    % \centering
    % \begin{tikzpicture}[
      % every path/.style=edgestyle
      % ]
      % Judges
      % \node[judge]                  (J1c)    {J1};
      % \node[judge, right=1cm of J1c] (J2c)    {J2};
      % \node[judge, right=1cm of J2c] (J3c)    {J3};
      % Latents
      % \node[quality, above=1cm of J2c, xshift=-0.8cm] (Qc) {Q};
      % \node[confounder, right=of Qc]                  (Cc) {C};
      % edges
      % \draw (Qc) -- (J1c) (Qc) -- (J2c) (Qc) -- (J3c);
      % \draw (Cc) -- (J1c) (Cc) -- (J2c) (Cc) -- (J3c);
      % \draw (J2c) -- (J3c);
    % \end{tikzpicture}
    % \caption{Confounder-aware (Ours)}
  % \end{subfigure}

% \caption{\textbf{Graphical models for aggregating judge scores under different structural assumptions.} \textbf{(a)} Naive model assumes scores reflect only a true latent quality (Q). \textbf{(b)} Connection-aware model includes direct inter-judge interactions. \textbf{(c)} Our Confounder-aware model introduces an additional latent confounder (C) influencing judge scores.}
% \label{fig:latent_subplots}
% \end{figure*}


==> figures/pgm_old.tex <==
\usetikzlibrary{positioning}

% pick a nice orange from the Tableau palette
\definecolor{tableauorange}{RGB}{237,125,49}

\tikzset{
  judge/.style={
    circle,
    draw=tableauorange!80!black,
    fill=tableauorange!30,
    minimum size=20pt,
    inner sep=1pt
  },
  quality/.style={
    circle,
    draw=blue!80!black,
    fill=blue!20,
    dashed,
    minimum size=20pt
  },
  confounder/.style={
    circle,
    draw=red!80!black,
    fill=red!20,
    dashed,
    minimum size=20pt
  },
  edgestyle/.style={thick}
}

\begin{figure*}[t]
  \centering
  % (a) Only true‐quality
  \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \begin{tikzpicture}[
      every path/.style=edgestyle
      ]
      % Judges
      \node[judge]  (J1a)               {J1};
      \node[judge, right=1cm of J1a] (J2a)               {J2};
      \node[judge, right=1cm of J2a] (J3a)            {J3};
      % latent Q
      \node[quality, above=1cm of J2a] (Q1)                {Q};
      % edges
      \draw (Q1) -- (J1a);
      \draw (Q1) -- (J2a);
      \draw (Q1) -- (J3a);
    \end{tikzpicture}
    \caption{Naive: only true‐quality}
  \end{subfigure}
  \hfill
  % (b) Connection‐aware
  \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \begin{tikzpicture}[
      every path/.style=edgestyle
      ]
      % Judges
      \node[judge]  (J1b)               {J1};
      \node[judge, right=1cm of J1b] (J2b)               {J2};
      \node[judge, right=1cm of J2b] (J3b)            {J3};
      % latent Q
      \node[quality, above=1cm of J2b] (Q2)                {Q};
      % edges
      \draw (Q2) -- (J1b);
      \draw (Q2) -- (J2b);
      \draw (Q2) -- (J3b);
      \draw (J2b) -- (J3b);
    \end{tikzpicture}
    \caption{Connection-aware}
  \end{subfigure}
  \hfill
  % (c) Confounder‐aware
  \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \begin{tikzpicture}[
      every path/.style=edgestyle
      ]
      % Judges
      \node[judge]                  (J1c)    {J1};
      \node[judge, right=1cm of J1c] (J2c)    {J2};
      \node[judge, right=1cm of J2c] (J3c)    {J3};
      % Latents
      \node[quality, above=1cm of J2c, xshift=-0.8cm] (Qc) {Q};
      \node[confounder, right=of Qc]                  (Cc) {C};
      % edges
      \draw (Qc) -- (J1c) (Qc) -- (J2c) (Qc) -- (J3c);
      \draw (Cc) -- (J1c) (Cc) -- (J2c) (Cc) -- (J3c);
      \draw (J2c) -- (J3c);
    \end{tikzpicture}
    \caption{Confounder-aware (Ours)}
  \end{subfigure}

  \caption{Graphical models for aggregating judge scores under different structural assumptions. 
    \textbf{(a)} Naive model: each judge score is driven only by a single latent quality factor, with no inter-judge links. 
    \textbf{(b)} Connection-aware model: adds direct links among judges. 
    \textbf{(c)} Confounder-aware model (ours): introduces a shared latent confounder $C$ in addition to the true‐quality $Q$.}
  \label{fig:latent_subplots}
\end{figure*}

==> sections/5_related_works.tex <==
\section{Related Work}
%
We discuss related work in \emph{bias in LLM-as-a-judge}, \emph{label aggregation}, and highlight our contribution.
%
An extended discussion is provided in Appendix~\ref{appsec:extended_related_work}.

\paragraph{Bias in LLM-as-a-judge.}
%
LLMs used as automated evaluators exhibit systematic preferences such as positional, verbosity, authority, and self‑enhancement biases~\citep{ye2025justice,zhujudgelm}.
%
To mitigate these issues, prior work has explored prompt-based interventions~\citep{shi2024judging,jiao2024enhancing,ye2025justice} and fine-tuned evaluators such as JudgeLM and PandaLM, which aims to align model judgments more closely with human preferences~\citep{zhujudgelm,wangpandalm,li-etal-2024-split}.
%
\textit{\textbf{While effective locally, these techniques debias each single LLM judge and do not address the downstream problem of aggregating multiple, potentially correlated, LLM scores.}}


\paragraph{Label Aggregation.} 
%
Classic aggregation models such as Dawid–Skene~\citep{dawid1979}, GLAD~\citep{whitehill2009glad}, and MACE~\citep{hovy2013mace} infer latent truth by modeling annotator‑specific error rates.
%
Weak supervision frameworks generalize this idea to programmatic sources~\citep{bach2018snorkel,fu2020fast, shin21universalizing}.
%
Recently, \citep{hu2024language} introduce GED, a framework that ensembles and denoises preference graphs from multiple weak LLM evaluators to produce consistent and reliable model rankings.
%
Additionally, \citet{wang2025improving} analyzed inference methods for LLM-as-a-judge, examining judge probability distributions and comparing pre- and post-aggregation effects on scores using statistics like mean and mode (i.e., greedy decoding).
%
\textit{\textbf{However, these methods do not account for shared confounding factors that systematically influence annotators or LLMs alike.}}


\paragraph{Our Contribution.} 
%
We propose the first \emph{confounder-aware aggregation} method for LLM-as-a-judge setting.
%
Unlike prior work that assumes independent annotator noise around a latent true score, our approach explicitly models shared latent confounders, such as verbosity or formality, that may jointly affect all judges.
%
This bridges the gap between single-judge bias mitigation and statistical aggregation, enabling more reliable consensus in the presence of correlated judgment errors.

==> sections/99_checklist.tex <==
\section*{Checklist}

\begin{enumerate}

  \item For all models and algorithms presented, check if you include:
  \begin{enumerate}
    \item A clear description of the mathematical setting, assumptions, algorithm, and/or model. [Yes], Section \ref{sec:theory} and Appendix \ref{appsec:theory}.
    \item An analysis of the properties and complexity (time, space, sample size) of any algorithm. [Yes], Section \ref{sec:theory} and Appendix \ref{appsec:theory}.
    \item (Optional) Anonymized source code, with specification of all dependencies, including external libraries. [Yes], supplemental material
  \end{enumerate}

  \item For any theoretical claim, check if you include:
  \begin{enumerate}
    \item Statements of the full set of assumptions of all theoretical results. [Yes], Section \ref{sec:theory} and Appendix \ref{appsec:theory}.
    \item Complete proofs of all theoretical results. [Yes], Section \ref{sec:theory} and Appendix \ref{appsec:theory}.
    \item Clear explanations of any assumptions. [Yes], Section \ref{sec:theory} and Appendix \ref{appsec:theory}.
  \end{enumerate}

  \item For all figures and tables that present empirical results, check if you include:
  \begin{enumerate}
    \item The code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL). [Yes], Supplementary
    \item All the training details (e.g., data splits, hyperparameters, how they were chosen). [Yes], Appendix \
    \item A clear definition of the specific measure or statistics and error bars (e.g., with respect to the random seed after running experiments multiple times). [Yes]
    \item A description of the computing infrastructure used. (e.g., type of GPUs, internal cluster, or cloud provider). [Yes], Appendix \ref{appsec:exp_details}
  \end{enumerate}

  \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets, check if you include:
  \begin{enumerate}
    \item Citations of the creator If your work uses existing assets. [Yes]
    \item The license information of the assets, if applicable. [Not Applicable]
    \item New assets either in the supplemental material or as a URL, if applicable. [Yes]
    \item Information about consent from data providers/curators. [Not Applicable]
    \item Discussion of sensible content if applicable, e.g., personally identifiable information or offensive content. [Not Applicable]
  \end{enumerate}

  \item If you used crowdsourcing or conducted research with human subjects, check if you include:
  \begin{enumerate}
    \item The full text of instructions given to participants and screenshots. [Not Applicable]
    \item Descriptions of potential participant risks, with links to Institutional Review Board (IRB) approvals if applicable. [Not Applicable]
    \item The estimated hourly wage paid to participants and the total amount spent on participant compensation. [Not Applicable]
  \end{enumerate}

\end{enumerate}



==> tables/binary_agg.tex <==
% \begin{table*}[t!]
% \caption{Aggregation performance across classification and preference datasets, measured by Accuracy. Higher values indicate better aggregation.}
% \label{tab:results_binary}
% \centering
% \sisetup{
%   round-mode=places,
%   round-precision=3,
%   table-format=1.4,
%   table-number-alignment=center
% }
% \small
% \begin{tabularx}{0.98\textwidth}{@{}l *{6}{S}@{}}
% \toprule
%  & \textbf{CivilComments} & \textbf{JudgeBench} & \textbf{PKU-BETTER} & \textbf{PKU-SAFER} & \textbf{SHP} & \textbf{MT-Bench} \\ 
% \midrule
% MV     & 0.7650 & 0.4740 & 0.7010 & 0.7040 & 0.7460 & 0.6350 \\
% AVG    & 0.7710 & 0.4580 & 0.7130 & 0.7190 & 0.6840 & 0.5730 \\
% WS     & 0.7690 & 0.5240 & 0.8010 & 0.7480 & 0.7940 & 0.6420 \\
% UWS    & 0.7680 & 0.4500 & 0.7210 & 0.7210 & 0.6870 & 0.5720 \\
% \midrule
% CARE-SVD & 0.7150 & \textbf{0.542} & 0.3210 & 0.6130 & 0.7640 & 0.6090 \\
% CARE-Tensor  & \textbf{0.776} & 0.5080 & \textbf{0.838} & \textbf{0.785} & \textbf{0.846} & \textbf{0.682} \\ 
% \bottomrule
% \end{tabularx}
% \end{table*}


\begin{table*}[t!]
\caption{Performance across classification and preference datasets for binary judges, measured by Accuracy ($\uparrow$). 
% Higher values indicate better aggregation.
}
\vspace{-8pt}
\label{tab:results_binary}
\centering
\small
\begin{tabular*}{0.98\textwidth}{@{\extracolsep{\fill}}lcccccc}
\toprule
& \textbf{CivilComments} & \textbf{JudgeBench} & \textbf{PKU-BETTER} & \textbf{PKU-SAFER} & \textbf{SHP} & \textbf{MT-Bench} \\
\midrule
MV          & 0.765 & 0.474 & 0.701 & 0.704 & 0.746 & 0.635 \\
AVG         & 0.771 & 0.458 & 0.713 & 0.719 & 0.684 & 0.573 \\
WS          & 0.769 & 0.524 & 0.801 & 0.748 & 0.794 & 0.642 \\
UWS         & 0.768 & 0.450 & 0.721 & 0.721 & 0.687 & 0.572 \\
\midrule
CARE-SVD    & 0.715 & \textbf{0.542} & 0.321 & 0.613 & 0.764 & 0.609 \\
CARE-Tensor & \textbf{0.776} & 0.508 & \textbf{0.838} & \textbf{0.785} & \textbf{0.846} & \textbf{0.682} \\
\bottomrule
\end{tabular*}
\end{table*}


==> tables/individual_judge_performance.tex <==
%%%%%%%%%%% Color-coded individual-judge results (alternating rows) %%%%%%%%%%%
% \begin{table*}[h]
% \caption{Individual Judge Performance in Section \ref{subsec:exp_improved_agg}}\label{tab:results_individual_judge}
% \centering
% \resizebox{0.8\textwidth}{!}{%
% \begin{tabular}{@{}c|cc|cc|cc@{}}
% \toprule
 % & \multicolumn{2}{c|}{\textbf{FeedbackQA}} &
   % \multicolumn{2}{c|}{\textbf{HelpSteer2}} &
   % \multicolumn{2}{c}{\textbf{UltraFeedback}} \\
% \cmidrule(l){2-7}
 % & \multicolumn{1}{c|}{\cellcolor{red!30}MAE ($\downarrow$)} & % \cellcolor{green!30}$\tau$ ($\uparrow$) &
   % \multicolumn{1}{c|}{\cellcolor{red!30}MAE ($\downarrow$)} & % \cellcolor{green!30}$\tau$ ($\uparrow$) &
   % \multicolumn{1}{c|}{\cellcolor{red!30}MAE ($\downarrow$)} & \cellcolor{green!30}$\tau$ ($\uparrow$) \\ \midrule
% gemma-3-1b-it                & \multicolumn{1}{c|}{\cellcolor{red!20}1.0073} & \cellcolor{green!20}0.2315 & \multicolumn{1}{c|}{\cellcolor{red!20}1.0666} & \cellcolor{green!20}0.0825 & \multicolumn{1}{c|}{\cellcolor{red!20}1.0606} & \cellcolor{green!20}0.1812 \\ 
% gemma-3-4b-it                & \multicolumn{1}{c|}{\textbf{\cellcolor{red!10}0.7578}} & \cellcolor{green!10}0.4537 & \multicolumn{1}{c|}{\cellcolor{red!10}0.9920} & \cellcolor{green!10}0.1402 & \multicolumn{1}{c|}{\cellcolor{red!10}0.8492} & \cellcolor{green!10}0.2309 \\ 
% Llama-3.1-8B-Instruct        & \multicolumn{1}{c|}{\cellcolor{red!20}0.8148} & \cellcolor{green!20}0.4341 & \multicolumn{1}{c|}{\cellcolor{red!20}1.1364} & \cellcolor{green!20}0.1261 & \multicolumn{1}{c|}{\cellcolor{red!20}0.8648} & \cellcolor{green!20}0.3194 \\ 
% Llama-3.2-1B                 & \multicolumn{1}{c|}{\cellcolor{red!10}1.2219} & \cellcolor{green!10}{-0.0525} & \multicolumn{1}{c|}{\cellcolor{red!10}1.0049} & \cellcolor{green!10}{-0.0132} & \multicolumn{1}{c|}{\cellcolor{red!10}1.0119} & \cellcolor{green!10}0.0752 \\ 
% Llama-3.2-3B                 & \multicolumn{1}{c|}{\cellcolor{red!20}1.0362} & \cellcolor{green!20}0.0051 & \multicolumn{1}{c|}{\cellcolor{red!20}0.9995} & \cellcolor{green!20}0.0251 & \multicolumn{1}{c|}{\cellcolor{red!20}1.1522} & \cellcolor{green!20}0.1648 \\ 
% Mistral-7B-Instruct-v0.3     & \multicolumn{1}{c|}{\cellcolor{red!10}1.0244} & \cellcolor{green!10}0.4539 & \multicolumn{1}{c|}{\cellcolor{red!10}1.0793} & \cellcolor{green!10}0.1116 & \multicolumn{1}{c|}{\cellcolor{red!10}0.8572} & \cellcolor{green!10}0.1735 \\ 
% Phi-4-mini-instruct          & \multicolumn{1}{c|}{\cellcolor{red!20}0.8082} & \cellcolor{green!20}\textbf{0.4557} & \multicolumn{1}{c|}{\cellcolor{red!20}1.0692} & \cellcolor{green!20}0.1576 & \multicolumn{1}{c|}{\cellcolor{red!20}0.8355} & \cellcolor{green!20}0.3147 \\ 
% Qwen3-0.6B                   & \multicolumn{1}{c|}{\cellcolor{red!10}1.0969} & \cellcolor{green!10}0.2073 & \multicolumn{1}{c|}{\cellcolor{red!10}1.1255} & \cellcolor{green!10}0.0370 & \multicolumn{1}{c|}{\cellcolor{red!10}1.0233} & \cellcolor{green!10}0.1254 \\ 
% Qwen3-1.7B                   & \multicolumn{1}{c|}{\cellcolor{red!20}1.1507} & \cellcolor{green!20}0.2485 & \multicolumn{1}{c|}{\cellcolor{red!20}1.0693} & \cellcolor{green!20}0.1049 & \multicolumn{1}{c|}{\cellcolor{red!20}1.1382} & \cellcolor{green!20}0.1926 \\ 
% Qwen3-4B                     & \multicolumn{1}{c|}{\cellcolor{red!10}1.0999} & \cellcolor{green!10}0.2854 & \multicolumn{1}{c|}{\textbf{\cellcolor{red!10}0.9675}} & \cellcolor{green!10}\textbf{0.2290} & \multicolumn{1}{c|}{\textbf{\cellcolor{red!10}0.7088}} & \cellcolor{green!10}\textbf{0.3921} \\ 
% Qwen3-8B                     & \multicolumn{1}{c|}{\cellcolor{red!20}1.0517} & \cellcolor{green!20}0.4417 & \multicolumn{1}{c|}{\textbf{\cellcolor{red!20}0.9675}} & \cellcolor{green!20}0.2094 & \multicolumn{1}{c|}{\cellcolor{red!20}0.7512} & \cellcolor{green!20}0.3140 \\ 
% \bottomrule
% \end{tabular}%
% }
% \end{table*}




\begin{table*}[h]
\caption{Performance of individual judges across datasets, as evaluated in Section~\ref{subsec:exp_improved_agg}.}
% Metrics include MAE (lower is better) and Kendall’s $\tau$ (higher is better).
\label{tab:results_individual_judge}
\centering
\sisetup{
  round-mode=places,
  round-precision=4,
  table-format=-1.4,
  table-number-alignment=center
}
\small
\begin{tabularx}{0.87\textwidth}{@{}X *{6}{S}@{}}
\toprule
 & \multicolumn{2}{c}{\textbf{FeedbackQA}} & \multicolumn{2}{c}{\textbf{HelpSteer2}} & \multicolumn{2}{c}{\textbf{UltraFeedback}} \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
 & {\cellcolor{blue!10}MAE ($\downarrow$)} & {\cellcolor{teal!10}$\tau$ ($\uparrow$)} & {\cellcolor{blue!10}MAE ($\downarrow$)} & {\cellcolor{teal!10}$\tau$ ($\uparrow$)} & {\cellcolor{blue!10}MAE ($\downarrow$)} & {\cellcolor{teal!10}$\tau$ ($\uparrow$)} \\ 
\midrule
gemma-3-1b-it           & {\cellcolor{blue!10}1.0073} & {\cellcolor{teal!10}0.2315} & {\cellcolor{blue!10}1.0666} & {\cellcolor{teal!10}0.0825} & {\cellcolor{blue!10}1.0606} & {\cellcolor{teal!10}0.1812} \\
gemma-3-4b-it           & {\cellcolor{blue!10}\textbf{0.7578}} & {\cellcolor{teal!10}0.4537} & {\cellcolor{blue!10}0.9920} & {\cellcolor{teal!10}0.1402} & {\cellcolor{blue!10}0.8492} & {\cellcolor{teal!10}0.2309} \\
Llama-3.1-8B-Instruct   & {\cellcolor{blue!10}0.8148} & {\cellcolor{teal!10}0.4341} & {\cellcolor{blue!10}1.1364} & {\cellcolor{teal!10}0.1261} & {\cellcolor{blue!10}0.8648} & {\cellcolor{teal!10}0.3194} \\
Llama-3.2-1B            & {\cellcolor{blue!10}1.2219} & {\cellcolor{teal!10}{-0.0525}} & {\cellcolor{blue!10}1.0049} & {\cellcolor{teal!10}{-0.0132}} & {\cellcolor{blue!10}1.0119} & {\cellcolor{teal!10}0.0752} \\
Llama-3.2-3B            & {\cellcolor{blue!10}1.0362} & {\cellcolor{teal!10}0.0051} & {\cellcolor{blue!10}0.9995} & {\cellcolor{teal!10}0.0251} & {\cellcolor{blue!10}1.1522} & {\cellcolor{teal!10}0.1648} \\
Mistral-7B-Instruct-v0.3 & {\cellcolor{blue!10}1.0244} & {\cellcolor{teal!10}0.4539} & {\cellcolor{blue!10}1.0793} & {\cellcolor{teal!10}0.1116} & {\cellcolor{blue!10}0.8572} & {\cellcolor{teal!10}0.1735} \\
Phi-4-mini-instruct     & {\cellcolor{blue!10}0.8082} & {\cellcolor{teal!10}\textbf{0.4557}} & {\cellcolor{blue!10}1.0692} & {\cellcolor{teal!10}0.1576} & {\cellcolor{blue!10}0.8355} & {\cellcolor{teal!10}0.3147} \\
Qwen3-0.6B              & {\cellcolor{blue!10}1.0969} & {\cellcolor{teal!10}0.2073} & {\cellcolor{blue!10}1.1255} & {\cellcolor{teal!10}0.0370} & {\cellcolor{blue!10}1.0233} & {\cellcolor{teal!10}0.1254} \\
Qwen3-1.7B              & {\cellcolor{blue!10}1.1507} & {\cellcolor{teal!10}0.2485} & {\cellcolor{blue!10}1.0693} & {\cellcolor{teal!10}0.1049} & {\cellcolor{blue!10}1.1382} & {\cellcolor{teal!10}0.1926} \\
Qwen3-4B                & {\cellcolor{blue!10}1.0999} & {\cellcolor{teal!10}0.2854} & {\cellcolor{blue!10}\textbf{0.9675}} & {\cellcolor{teal!10}\textbf{0.2290}} & {\cellcolor{blue!10}\textbf{0.7088}} & {\cellcolor{teal!10}\textbf{0.3921}} \\
Qwen3-8B                & {\cellcolor{blue!10}1.0517} & {\cellcolor{teal!10}0.4417} & {\cellcolor{blue!10}\textbf{0.9675}} & {\cellcolor{teal!10}0.2094} & {\cellcolor{blue!10}0.7512} & {\cellcolor{teal!10}0.3140} \\
\bottomrule
\end{tabularx}
\end{table*}


==> tables/individual_program_judge_performance.tex <==
%%%%%%%%%%% Color-coded program-judge results (alternating rows) %%%%%%%%%%%
% \begin{table*}[h]
% \caption{Program Judge Performance. (*) represents the selected judges in Section \ref{subsec:exp_effective_integ_program_judges}.}\label{tab:results_individual_program_judges_performance}
% \centering
% \resizebox{0.9\textwidth}{!}{%
% \begin{tabular}{@{}c|cc|cc|cc@{}}
% \toprule
 % & \multicolumn{2}{c|}{\textbf{FeedbackQA}} &
   % \multicolumn{2}{c|}{\textbf{HelpSteer2}} &
   % \multicolumn{2}{c}{\textbf{UltraFeedback}} \\
% \cmidrule(l){2-7}
 % & \multicolumn{1}{c|}{\cellcolor{red!30}MAE ($\downarrow$)} & \cellcolor{green!30}$\tau$ ($\uparrow$) &
   % \multicolumn{1}{c|}{\cellcolor{red!30}MAE ($\downarrow$)} & \cellcolor{green!30}$\tau$ ($\uparrow$) &
   % \multicolumn{1}{c|}{\cellcolor{red!30}MAE ($\downarrow$)} & \cellcolor{green!30}$\tau$ ($\uparrow$) \\ \midrule
% factuality\_check\_score (*)                  & \multicolumn{1}{c|}{\cellcolor{red!20}1.9956} & \cellcolor{green!20}0.0872 & \multicolumn{1}{c|}{\cellcolor{red!20}1.1992} & \cellcolor{green!20}0.0075 & \multicolumn{1}{c|}{\cellcolor{red!20}1.1910} & \cellcolor{green!20}0.0492 \\
% factuality\_factKB\_score (*)                 & \multicolumn{1}{c|}{\cellcolor{red!10}1.0343} & \cellcolor{green!10}0.2288 & \multicolumn{1}{c|}{\cellcolor{red!10}1.7180} & \cellcolor{green!10}0.0414 & \multicolumn{1}{c|}{\cellcolor{red!10}1.4342} & \cellcolor{green!10}0.1051 \\ 
% readability\_flesch\_reading  (*)            & \multicolumn{1}{c|}{\cellcolor{red!20}1.2185} & \cellcolor{green!20}0.0431 & \multicolumn{1}{c|}{\cellcolor{red!20}2.5682} & \cellcolor{green!20}0.0445 & \multicolumn{1}{c|}{\cellcolor{red!20}2.5145} & \cellcolor{green!20}0.1396 \\ 
% readability\_smog (*)                       & \multicolumn{1}{c|}{\cellcolor{red!10}0.9805} & \cellcolor{green!10}0.1277 & \multicolumn{1}{c|}{\cellcolor{red!10}2.3286} & \cellcolor{green!10}0.0283 & \multicolumn{1}{c|}{\cellcolor{red!10}2.3122} & \cellcolor{green!10}0.1604 \\ 
% relevance\_bleu                          & \multicolumn{1}{c|}{\cellcolor{red!20}1.4035} & \cellcolor{green!20}0.0126 & \multicolumn{1}{c|}{\cellcolor{red!20}2.7452} & \cellcolor{green!20}{-0.0355} & \multicolumn{1}{c|}{\cellcolor{red!20}2.7330} & \cellcolor{green!20}0.0560 \\ 
% relevance\_keyword\_overlap               & \multicolumn{1}{c|}{\cellcolor{red!10}1.2779} & \cellcolor{green!10}0.1977 & \multicolumn{1}{c|}{\cellcolor{red!10}2.3735} & \cellcolor{green!10}0.0138 & \multicolumn{1}{c|}{\cellcolor{red!10}2.2725} & \cellcolor{green!10}0.1461 \\ 
% relevance\_lexical\_overlap (*)              & \multicolumn{1}{c|}{\cellcolor{red!20}1.1371} & \cellcolor{green!20}0.2316 & \multicolumn{1}{c|}{\cellcolor{red!20}2.0148} & \cellcolor{green!20}{-0.0144} & \multicolumn{1}{c|}{\cellcolor{red!20}1.9182} & \cellcolor{green!20}0.1187 \\ 
% relevance\_rouge                         & \multicolumn{1}{c|}{\cellcolor{red!10}1.3079} & \cellcolor{green!10}0.2066 & \multicolumn{1}{c|}{\cellcolor{red!10}2.5603} & \cellcolor{green!10}0.0232 & \multicolumn{1}{c|}{\cellcolor{red!10}2.4838} & \cellcolor{green!10}0.1327 \\ 
% relevance\_semantic\_sim\_strong (*)           & \multicolumn{1}{c|}{\textbf{\cellcolor{red!20}0.8759}} & \textbf{\cellcolor{green!20}0.4092} & \multicolumn{1}{c|}{\cellcolor{red!20}1.1182} & \cellcolor{green!20}0.0395 & \multicolumn{1}{c|}{\textbf{\cellcolor{red!20}0.9866}} & \cellcolor{green!20}0.1601 \\ 
% safety\_toxicity (*)                         & \multicolumn{1}{c|}{\cellcolor{red!10}1.5396} & \cellcolor{green!10}{-0.0380} & \multicolumn{1}{c|}{\textbf{\cellcolor{red!10}1.1105}} & \cellcolor{green!10}0.0300 & \multicolumn{1}{c|}{\cellcolor{red!10}1.0139} & \cellcolor{green!10}{-0.0043} \\ 
% structure\_avg\_paragraph\_length\_dist     & \multicolumn{1}{c|}{\cellcolor{red!20}1.4560} & \cellcolor{green!20}{-0.1883} & \multicolumn{1}{c|}{\cellcolor{red!20}2.5562} & \cellcolor{green!20}{-0.0081} & \multicolumn{1}{c|}{\cellcolor{red!20}2.4637} & \cellcolor{green!20}0.1074 \\ 
% structure\_avg\_sentence\_length\_dist      & \multicolumn{1}{c|}{\cellcolor{red!10}1.5248} & \cellcolor{green!10}{-0.0140} & \multicolumn{1}{c|}{\cellcolor{red!10}2.4407} & \cellcolor{green!10}{-0.0287} & \multicolumn{1}{c|}{\cellcolor{red!10}2.4179} & \cellcolor{green!10}0.1612 \\ 
% structure\_cohesion\_score                & \multicolumn{1}{c|}{\cellcolor{red!20}1.4078} & \cellcolor{green!20}0.2070 & \multicolumn{1}{c|}{\cellcolor{red!20}2.7139} & \cellcolor{green!20}0.0345 & \multicolumn{1}{c|}{\cellcolor{red!20}2.6578} & \cellcolor{green!20}0.1567 \\ 
% structure\_emphasis\_count                & \multicolumn{1}{c|}{\cellcolor{red!10}1.2826} & \cellcolor{green!10}0.1988 & \multicolumn{1}{c|}{\cellcolor{red!10}2.6642} & \cellcolor{green!10}0.0482 & \multicolumn{1}{c|}{\cellcolor{red!10}2.5955} & \cellcolor{green!10}0.2060 \\ 
% structure\_headings                      & \multicolumn{1}{c|}{\cellcolor{red!20}1.4765} & \cellcolor{green!20}0.0423 & \multicolumn{1}{c|}{\cellcolor{red!20}2.6521} & \cellcolor{green!20}{-0.0340} & \multicolumn{1}{c|}{\cellcolor{red!20}2.5916} & \cellcolor{green!20}0.1049 \\ 
% structure\_lexical\_diversity             & \multicolumn{1}{c|}{\cellcolor{red!10}1.0672} & \cellcolor{green!10}0.1625 & \multicolumn{1}{c|}{\cellcolor{red!10}2.1864} & \cellcolor{green!10}0.0444 & \multicolumn{1}{c|}{\cellcolor{red!10}2.0981} & \cellcolor{green!10}0.1935 \\ 
% structure\_list\_usage                    & \multicolumn{1}{c|}{\cellcolor{red!20}1.6284} & \cellcolor{green!20}0.0159 & \multicolumn{1}{c|}{\cellcolor{red!20}3.0208} & \cellcolor{green!20}{-0.0108} & \multicolumn{1}{c|}{\cellcolor{red!20}3.0132} & \cellcolor{green!20}0.0872 \\ 
% structure\_logical\_transitions (*)           & \multicolumn{1}{c|}{\cellcolor{red!10}1.2694} & \cellcolor{green!10}0.1743 & \multicolumn{1}{c|}{\cellcolor{red!10}2.2693} & \cellcolor{green!10}0.0520 & \multicolumn{1}{c|}{\cellcolor{red!10}2.4355} & \cellcolor{green!10}0.2263 \\ 
% structure\_max\_sentence\_length (*)          & \multicolumn{1}{c|}{\cellcolor{red!20}1.3039} & \cellcolor{green!20}0.1272 & \multicolumn{1}{c|}{\cellcolor{red!20}2.7532} & \cellcolor{green!20}0.0104 & \multicolumn{1}{c|}{\cellcolor{red!20}2.7511} & \cellcolor{green!20}0.1377 \\ 
% structure\_min\_sentence\_length           & \multicolumn{1}{c|}{\cellcolor{red!10}1.3568} & \cellcolor{green!10}0.1887 & \multicolumn{1}{c|}{\cellcolor{red!10}2.4872} & \cellcolor{green!10}0.0400 & \multicolumn{1}{c|}{\cellcolor{red!10}2.4322} & \cellcolor{green!10}0.2046 \\ 
% structure\_questions                     & \multicolumn{1}{c|}{\cellcolor{red!20}1.2443} & \cellcolor{green!20}0.2692 & \multicolumn{1}{c|}{\cellcolor{red!20}2.4910} & \cellcolor{green!20}0.0360 & \multicolumn{1}{c|}{\cellcolor{red!20}2.4064} & \cellcolor{green!20}0.2114 \\ 
% structure\_sentence\_balance              & \multicolumn{1}{c|}{\cellcolor{red!10}1.4423} & \cellcolor{green!10}0.1835 & \multicolumn{1}{c|}{\cellcolor{red!10}2.6757} & \cellcolor{green!10}0.0501 & \multicolumn{1}{c|}{\cellcolor{red!10}2.6444} & \cellcolor{green!10}0.2203 \\ 
% structure\_sentence\_count (*)                & \multicolumn{1}{c|}{\cellcolor{red!20}1.3099} & \cellcolor{green!20}0.1742 & \multicolumn{1}{c|}{\cellcolor{red!20}2.4408} & \textbf{\cellcolor{green!20}0.0807} & \multicolumn{1}{c|}{\cellcolor{red!20}2.6570} & \textbf{\cellcolor{green!20}0.2300} \\ 

% \end{tabular}%
% }
% \end{table*}




\begin{table*}[h!]
\caption{Performance of individual program judges across datasets, with (*) indicating judges selected in Section~\ref{subsec:exp_effective_integ_program_judges}.}
\label{tab:results_individual_program_judges_performance}
\centering
\sisetup{
  round-mode=places,
  round-precision=4,
  table-format=-1.4,
  table-number-alignment=center
}
\small
\begin{tabularx}{\textwidth}{@{}X *{6}{S}@{}}
\toprule
 & \multicolumn{2}{c}{\textbf{FeedbackQA}} & \multicolumn{2}{c}{\textbf{HelpSteer2}} & \multicolumn{2}{c}{\textbf{UltraFeedback}} \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
 & {\cellcolor{blue!10}MAE ($\downarrow$)} & {\cellcolor{teal!10}$\tau$ ($\uparrow$)} & {\cellcolor{blue!10}MAE ($\downarrow$)} & {\cellcolor{teal!10}$\tau$ ($\uparrow$)} & {\cellcolor{blue!10}MAE ($\downarrow$)} & {\cellcolor{teal!10}$\tau$ ($\uparrow$)} \\ 
\midrule
factuality\_check\_score (*)           & {\cellcolor{blue!10}1.9956} & {\cellcolor{teal!10}0.0872} & {\cellcolor{blue!10}1.1992} & {\cellcolor{teal!10}0.0075} & {\cellcolor{blue!10}1.1910} & {\cellcolor{teal!10}0.0492} \\
factuality\_factKB\_score (*)          & {\cellcolor{blue!10}1.0343} & {\cellcolor{teal!10}0.2288} & {\cellcolor{blue!10}1.7180} & {\cellcolor{teal!10}0.0414} & {\cellcolor{blue!10}1.4342} & {\cellcolor{teal!10}0.1051} \\
readability\_flesch\_reading (*)       & {\cellcolor{blue!10}1.2185} & {\cellcolor{teal!10}0.0431} & {\cellcolor{blue!10}2.5682} & {\cellcolor{teal!10}0.0445} & {\cellcolor{blue!10}2.5145} & {\cellcolor{teal!10}0.1396} \\
readability\_smog (*)                  & {\cellcolor{blue!10}0.9805} & {\cellcolor{teal!10}0.1277} & {\cellcolor{blue!10}2.3286} & {\cellcolor{teal!10}0.0283} & {\cellcolor{blue!10}2.3122} & {\cellcolor{teal!10}0.1604} \\
relevance\_bleu                        & {\cellcolor{blue!10}1.4035} & {\cellcolor{teal!10}0.0126} & {\cellcolor{blue!10}2.7452} & {\cellcolor{teal!10}{-0.0355}} & {\cellcolor{blue!10}2.7330} & {\cellcolor{teal!10}0.0560} \\
relevance\_keyword\_overlap            & {\cellcolor{blue!10}1.2779} & {\cellcolor{teal!10}0.1977} & {\cellcolor{blue!10}2.3735} & {\cellcolor{teal!10}0.0138} & {\cellcolor{blue!10}2.2725} & {\cellcolor{teal!10}0.1461} \\
relevance\_lexical\_overlap (*)        & {\cellcolor{blue!10}1.1371} & {\cellcolor{teal!10}0.2316} & {\cellcolor{blue!10}2.0148} & {\cellcolor{teal!10}{-0.0144}} & {\cellcolor{blue!10}1.9182} & {\cellcolor{teal!10}0.1187} \\
relevance\_rouge                       & {\cellcolor{blue!10}1.3079} & {\cellcolor{teal!10}0.2066} & {\cellcolor{blue!10}2.5603} & {\cellcolor{teal!10}0.0232} & {\cellcolor{blue!10}2.4838} & {\cellcolor{teal!10}0.1327} \\
relevance\_semantic\_sim\_strong (*)   & {\cellcolor{blue!10}\textbf{0.8759}} & {\cellcolor{teal!10}\textbf{0.4092}} & {\cellcolor{blue!10}1.1182} & {\cellcolor{teal!10}0.0395} & {\cellcolor{blue!10}\textbf{0.9866}} & {\cellcolor{teal!10}0.1601} \\
safety\_toxicity (*)                   & {\cellcolor{blue!10}1.5396} & {\cellcolor{teal!10}{-0.0380}} & {\cellcolor{blue!10}\textbf{1.1105}} & {\cellcolor{teal!10}0.0300} & {\cellcolor{blue!10}1.0139} & {\cellcolor{teal!10}{-0.0043}} \\
structure\_avg\_paragraph\_length\_dist & {\cellcolor{blue!10}1.4560} & {\cellcolor{teal!10}{-0.1883}} & {\cellcolor{blue!10}2.5562} & {\cellcolor{teal!10}{-0.0081}} & {\cellcolor{blue!10}2.4637} & {\cellcolor{teal!10}0.1074} \\
structure\_avg\_sentence\_length\_dist & {\cellcolor{blue!10}1.5248} & {\cellcolor{teal!10}{-0.0140}} & {\cellcolor{blue!10}2.4407} & {\cellcolor{teal!10}{-0.0287}} & {\cellcolor{blue!10}2.4179} & {\cellcolor{teal!10}0.1612} \\
structure\_cohesion\_score             & {\cellcolor{blue!10}1.4078} & {\cellcolor{teal!10}0.2070} & {\cellcolor{blue!10}2.7139} & {\cellcolor{teal!10}0.0345} & {\cellcolor{blue!10}2.6578} & {\cellcolor{teal!10}0.1567} \\
structure\_emphasis\_count             & {\cellcolor{blue!10}1.2826} & {\cellcolor{teal!10}0.1988} & {\cellcolor{blue!10}2.6642} & {\cellcolor{teal!10}0.0482} & {\cellcolor{blue!10}2.5955} & {\cellcolor{teal!10}0.2060} \\
structure\_headings                    & {\cellcolor{blue!10}1.4765} & {\cellcolor{teal!10}0.0423} & {\cellcolor{blue!10}2.6521} & {\cellcolor{teal!10}{-0.0340}} & {\cellcolor{blue!10}2.5916} & {\cellcolor{teal!10}0.1049} \\
structure\_lexical\_diversity          & {\cellcolor{blue!10}1.0672} & {\cellcolor{teal!10}0.1625} & {\cellcolor{blue!10}2.1864} & {\cellcolor{teal!10}0.0444} & {\cellcolor{blue!10}2.0981} & {\cellcolor{teal!10}0.1935} \\
structure\_list\_usage                 & {\cellcolor{blue!10}1.6284} & {\cellcolor{teal!10}0.0159} & {\cellcolor{blue!10}3.0208} & {\cellcolor{teal!10}{-0.0108}} & {\cellcolor{blue!10}3.0132} & {\cellcolor{teal!10}0.0872} \\
structure\_logical\_transitions (*)    & {\cellcolor{blue!10}1.2694} & {\cellcolor{teal!10}0.1743} & {\cellcolor{blue!10}2.2693} & {\cellcolor{teal!10}0.0520} & {\cellcolor{blue!10}2.4355} & {\cellcolor{teal!10}0.2263} \\
structure\_max\_sentence\_length (*)   & {\cellcolor{blue!10}1.3039} & {\cellcolor{teal!10}0.1272} & {\cellcolor{blue!10}2.7532} & {\cellcolor{teal!10}0.0104} & {\cellcolor{blue!10}2.7511} & {\cellcolor{teal!10}0.1377} \\
structure\_min\_sentence\_length       & {\cellcolor{blue!10}1.3568} & {\cellcolor{teal!10}0.1887} & {\cellcolor{blue!10}2.4872} & {\cellcolor{teal!10}0.0400} & {\cellcolor{blue!10}2.4322} & {\cellcolor{teal!10}0.2046} \\
structure\_questions                   & {\cellcolor{blue!10}1.2443} & {\cellcolor{teal!10}0.2692} & {\cellcolor{blue!10}2.4910} & {\cellcolor{teal!10}0.0360} & {\cellcolor{blue!10}2.4064} & {\cellcolor{teal!10}0.2114} \\
structure\_sentence\_balance           & {\cellcolor{blue!10}1.4423} & {\cellcolor{teal!10}0.1835} & {\cellcolor{blue!10}2.6757} & {\cellcolor{teal!10}0.0501} & {\cellcolor{blue!10}2.6444} & {\cellcolor{teal!10}0.2203} \\
structure\_sentence\_count (*)         & {\cellcolor{blue!10}1.3099} & {\cellcolor{teal!10}0.1742} & {\cellcolor{blue!10}2.4408} & {\cellcolor{teal!10}\textbf{0.0807}} & {\cellcolor{blue!10}2.6570} & {\cellcolor{teal!10}\textbf{0.2300}} \\
\bottomrule
\end{tabularx}
\end{table*}

==> tables/intervention.tex <==
%%%%%%%%%%%% Gray color table %%%%%%%%%%
% \begin{table*}[t!]
% \caption{Comparison with aggregation methods using individually intervened LLM judges. While other baselines aggregate scores from debiased LLM judges, \textsc{CARE} operates directly on raw outputs. 
% %Lower MAE and higher Kendall’s $\tau$ indicate better performance.
% }\label{tab:results_intervention}
% \centering
% \resizebox{0.6\textwidth}{!}{%
% \begin{tabular}{@{}c|cc|cc|cc@{}}
% \toprule
%  & \multicolumn{2}{c|}{\textbf{FeedbackQA}} & \multicolumn{2}{c|}{\textbf{HelpSteer2}} & \multicolumn{2}{c}{\textbf{UltraFeedback}} \\ \cmidrule(l){2-7} 
%  & \multicolumn{1}{c|}{MAE ($\downarrow$)} & $\tau$ ($\uparrow$) & \multicolumn{1}{c|}{MAE ($\downarrow$)} & $\tau$ ($\uparrow$) & \multicolumn{1}{c|}{MAE ($\downarrow$)} & $\tau$ ($\uparrow$) \\ \midrule
% \rowcolor[HTML]{EFEFEF} 
% MV & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.8004} & 0.9640 & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.9951} & 0.1629 & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.8562} & 0.2799 \\
% AVG & \multicolumn{1}{c|}{0.8029} & 0.4412 & \multicolumn{1}{c|}{0.9822} & 0.1611 & \multicolumn{1}{c|}{0.6801} & 0.3704 \\
% \rowcolor[HTML]{EFEFEF} 
% WS & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{0.7674}} & 0.4429 & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}1.3030} & 0.1511 & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}1.1516} & 0.3588 \\
% UWS & \multicolumn{1}{c|}{0.8117} & 0.4390 & \multicolumn{1}{c|}{0.9849} & 0.1697 & \multicolumn{1}{c|}{0.6683} & 0.3782 \\
% \rowcolor[HTML]{EFEFEF} 
% CARE & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.7866} & \textbf{0.4542} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{0.9742}} & \textbf{0.1805} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{0.6379}} & \textbf{0.3806} \\ \bottomrule
% \end{tabular}%
% }
% \end{table*}

%%%%%%%%%%% Colorify tables %%%%%%%%%%
% \begin{table*}[t!]
% \caption{Comparison with aggregation methods using individually intervened LLM judges. While other baselines aggregate scores from debiased LLM judges, \textsc{CARE} operates directly on raw outputs. 
%Lower MAE and higher Kendall’s $\tau$ indicate better performance.
% }\label{tab:results_intervention}
% \centering
% \resizebox{0.6\textwidth}{!}{%
% \begin{tabular}{@{}c|cc|cc|cc@{}}
% \toprule
 % & \multicolumn{2}{c|}{\textbf{FeedbackQA}} & \multicolumn{2}{c|}{\textbf{HelpSteer2}} & \multicolumn{2}{c}{\textbf{UltraFeedback}} \\ \cmidrule(l){2-7} 
 % & \multicolumn{1}{c|}{\cellcolor{red!30}MAE ($\downarrow$)} & \cellcolor{green!30}$\tau$ ($\uparrow$) & \multicolumn{1}{c|}{\cellcolor{red!30}MAE ($\downarrow$)} & \cellcolor{green!30}$\tau$ ($\uparrow$) & \multicolumn{1}{c|}{\cellcolor{red!30}MAE ($\downarrow$)} & \cellcolor{green!30}$\tau$ ($\uparrow$) \\ \midrule

% MV & \multicolumn{1}{c|}{\cellcolor{red!20}0.8004} & \cellcolor{green!20}0.9640 & \multicolumn{1}{c|}{\cellcolor{red!20}0.9951} & \cellcolor{green!20}0.1629 & \multicolumn{1}{c|}{\cellcolor{red!20}0.8562} & \cellcolor{green!20}0.2799 \\

% AVG & \multicolumn{1}{c|}{\cellcolor{red!10}0.8029} & \cellcolor{green!10}0.4412 & \multicolumn{1}{c|}{\cellcolor{red!10}0.9822} & \cellcolor{green!10}0.1611 & \multicolumn{1}{c|}{\cellcolor{red!10}0.6801} & \cellcolor{green!10}0.3704 \\

% WS & \multicolumn{1}{c|}{\textbf{\cellcolor{red!20}0.7674}} & \cellcolor{green!20}0.4429 & \multicolumn{1}{c|}{\cellcolor{red!20}1.3030} & \cellcolor{green!20}0.1511 & \multicolumn{1}{c|}{\cellcolor{red!20}1.1516} & \cellcolor{green!20}0.3588 \\

% UWS & \multicolumn{1}{c|}{\cellcolor{red!10}0.8117} & \cellcolor{green!10}0.4390 & \multicolumn{1}{c|}{\cellcolor{red!10}0.9849} & \cellcolor{green!10}0.1697 & \multicolumn{1}{c|}{\cellcolor{red!10}0.6683} & \cellcolor{green!10}0.3782 \\

% CARE & \multicolumn{1}{c|}{\cellcolor{red!20}0.7866} & \textbf{\cellcolor{green!20}0.4542} & \multicolumn{1}{c|}{\textbf{\cellcolor{red!20}0.9742}} & \textbf{\cellcolor{green!20}0.1805} & \multicolumn{1}{c|}{\textbf{\cellcolor{red!20}0.6379}} & \textbf{\cellcolor{green!20}0.3806} \\ \bottomrule
% \end{tabular}%
% }
% \end{table*}



\begin{table*}[t!]
\caption{Comparison of aggregation methods using individually intervened LLM judges. While other baselines aggregate scores from debiased LLM judges, \textsc{CARE} operates directly on raw outputs.}
\label{tab:results_intervention}
\centering
\sisetup{
  round-mode=places,
  round-precision=4,
  table-format=1.4,
  table-number-alignment=center
}
\small
\begin{tabularx}{0.69\textwidth}{@{}l *{6}{S}@{}}
\toprule
 & \multicolumn{2}{c}{\textbf{FeedbackQA}} & \multicolumn{2}{c}{\textbf{HelpSteer2}} & \multicolumn{2}{c}{\textbf{UltraFeedback}} \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
 & {\cellcolor{blue!10}MAE ($\downarrow$)} & {\cellcolor{teal!10}$\tau$ ($\uparrow$)} & {\cellcolor{blue!10}MAE ($\downarrow$)} & {\cellcolor{teal!10}$\tau$ ($\uparrow$)} & {\cellcolor{blue!10}MAE ($\downarrow$)} & {\cellcolor{teal!10}$\tau$ ($\uparrow$)} \\ 
\midrule
MV   & {\cellcolor{blue!10}0.8004} & {\cellcolor{teal!10}0.3964} & {\cellcolor{blue!10}0.9951} & {\cellcolor{teal!10}0.1629} & {\cellcolor{blue!10}0.8562} & {\cellcolor{teal!10}0.2799} \\
AVG  & {\cellcolor{blue!10}0.8029} & {\cellcolor{teal!10}0.4412} & {\cellcolor{blue!10}0.9822} & {\cellcolor{teal!10}0.1611} & {\cellcolor{blue!10}0.6801} & {\cellcolor{teal!10}0.3704} \\
WS   & {\cellcolor{blue!10}\textbf{0.7674}} & {\cellcolor{teal!10}0.4429} & {\cellcolor{blue!10}1.3030} & {\cellcolor{teal!10}0.1511} & {\cellcolor{blue!10}1.1516} & {\cellcolor{teal!10}0.3588} \\
UWS  & {\cellcolor{blue!10}0.8117} & {\cellcolor{teal!10}0.4390} & {\cellcolor{blue!10}0.9849} & {\cellcolor{teal!10}0.1697} & {\cellcolor{blue!10}0.6683} & {\cellcolor{teal!10}0.3782} \\
CARE & {\cellcolor{blue!10}0.7866} & {\cellcolor{teal!10}\textbf{0.4542}} & {\cellcolor{blue!10}\textbf{0.9742}} & {\cellcolor{teal!10}\textbf{0.1805}} & {\cellcolor{blue!10}\textbf{0.6379}} & {\cellcolor{teal!10}\textbf{0.3806}} \\ 
\bottomrule
\end{tabularx}
\end{table*}


==> tables/intervention_old.tex <==
\begin{table*}[t]
  \centering
  \begin{minipage}[t]{0.32\textwidth}
    \centering
    \caption*{\textbf{FeedbackQA}}
    \begin{tabular}{lrr}
      \toprule
       & MAE ($\downarrow$) & $\tau$ ($\uparrow$)\\
      \midrule
      MV   & 0.8004 & 0.964 \\
      AVG  & 0.8029 & 0.4412 \\
      WS   & \textbf{0.7674} & 0.4429 \\
      UWS  & 0.8117 & 0.4390 \\
      CARE & 0.7866 & \textbf{0.4542} \\
      \bottomrule
    \end{tabular}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.32\textwidth}
    \centering
    \caption*{\textbf{HelpSteer2}}
    \begin{tabular}{lrr}
      \toprule
      & MAE ($\downarrow$) & $\tau$ ($\uparrow$)\\
      \midrule
      MV   & 0.9951 & 0.1629 \\
      AVG  & 0.9822 & 0.1611 \\
      WS   & 1.3030 & 0.1511 \\
      UWS  & 0.9849 & 0.1697 \\
      CARE & \textbf{0.9742} & \textbf{0.1805} \\
      \bottomrule
    \end{tabular}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.32\textwidth}
    \centering
    \caption*{\textbf{UltraFeedback}}
    \begin{tabular}{lrr}
      \toprule
      & MAE ($\downarrow$) & $\tau$ ($\uparrow$)\\
      \midrule
      MV   & 0.8562 & 0.2799 \\
      AVG  & 0.6801 & 0.3704 \\
      WS   & 1.1516 & 0.3588 \\
      UWS  & 0.6683 & 0.3782 \\
      CARE & \textbf{0.6379} & \textbf{0.3860} \\
      \bottomrule
    \end{tabular}
  \end{minipage}
\caption{Comparison with aggregation methods using individually intervened LLM judges. While other baselines aggregate scores from debiased LLM judges, \textsc{CARE} operates directly on raw outputs. Lower MAE and higher Kendall’s $\tau$ indicate better performance.}\label{tab:results_intervention}
  
\end{table*}


==> tables/robustness_to_confounding_factors_old.tex <==

\begin{table}[t!]
  \centering
  \caption{Robustness to artificially injected bias. In each setting, a specific type of bias is introduced into system answers via prompting, and we evaluate the difference in aggregation scores before and after bias injection. \SYSNAME{} is particularly effective against stylistic biases such as beauty (rich content) and authority, but less effective for gender and fallacy biases, which may impact the actual quality of system answers.}\label{tab:robustness_to_confounding_factors}
  % tighten column spacing
  \setlength{\tabcolsep}{4pt}
  \begin{subtable}[t]{0.48\textwidth}
    \centering
    \caption{MAE ($\downarrow$)}
    \begin{adjustbox}{max width=\linewidth}
      \begin{tabular}{lcccc}
        \toprule
         & Beauty & Fallacy & Gender & Authority \\
        \midrule
        MV   & 0.9190 & 1.8971 & 1.7428 & 0.8239 \\
        AVG  & 0.5063 & 1.4007 & 1.1355 & 0.3250 \\
        WS   & 1.9225 & 2.5588 & 2.0217 & 0.9296 \\
        UWS  & 0.5080 & 1.3826 & 1.1646 & 0.2705 \\
        CARE & 0.3749 & 1.8996 & 1.5985 & 0.2466 \\
        \bottomrule
      \end{tabular}
    \end{adjustbox}
  \end{subtable}%
  \hfill
  \begin{subtable}[t]{0.48\textwidth}
    \centering
    \caption{Kendall's $\tau$ ($\uparrow$)}
    \begin{adjustbox}{max width=\linewidth}
      \begin{tabular}{lcccc}
        \toprule
         & Beauty & Fallacy & Gender & Authority \\
        \midrule
        MV   & 0.3336 & -0.0284 & 0.1272 & 0.2977 \\
        AVG  & 0.3943 &  0.1181 & 0.2879 & 0.4288 \\
        WS   & 0.3792 &  0.0680 & 0.2474 & 0.4886 \\
        UWS  & 0.4383 &  0.0491 & 0.2576 & 0.5799 \\
        CARE & 0.5323 &  0.0116 & 0.2311 & 0.6327 \\
        \bottomrule
      \end{tabular}

    \end{adjustbox}
  \end{subtable}
\end{table}



==> tables/score_agg_old.tex <==
\begin{table*}[t]
  \centering

  \begin{minipage}[t]{0.32\textwidth}
    \centering
    \caption*{\textbf{FeedbackQA}}
    \begin{tabular}{lrr}
      \toprule
       & MAE ($\downarrow$) & $\tau$ ($\uparrow$)\\
      \midrule
      MV   & 0.8812 & 0.3703 \\
      AVG  & 0.8492 & 0.4497 \\
      WS   & 0.8144 & 0.4401 \\
      UWS  & 0.9051 & \textbf{0.4580} \\
      CARE & \textbf{0.7866} & 0.4542 \\
      \bottomrule
    \end{tabular}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.32\textwidth}
    \centering
    \caption*{\textbf{HelpSteer2}}
    \begin{tabular}{lrr}
      \toprule
      & MAE ($\downarrow$) & $\tau$ ($\uparrow$)\\
      \midrule
      MV   & 0.9951 & 0.1629 \\
      AVG  & 0.9822 & 0.1611 \\
      WS   & 1.3030 & 0.1511 \\
      UWS  & 0.9849 & 0.1697 \\
      CARE & \textbf{0.9742} & \textbf{0.1805} \\
      \bottomrule
    \end{tabular}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.32\textwidth}
    \centering
    \caption*{\textbf{UltraFeedback}}
    \begin{tabular}{lrr}
      \toprule
      & MAE ($\downarrow$) & $\tau$ ($\uparrow$)\\
      \midrule
      MV   & 0.8522 & 0.2985 \\
      AVG  & 0.6860 & 0.3621 \\
      WS   & 1.1603 & 0.3306 \\
      UWS  & 0.6794 & 0.3669 \\
      CARE & \textbf{0.6379} & \textbf{0.3860} \\
      \bottomrule
    \end{tabular}
  \end{minipage}

  \caption{Aggregation performance across different datasets, measured by MAE (lower is better) and Kendall’s $\tau$ (higher is better). $\SYSNAME$ outperforms baseline methods in most cases.}
  \label{tab:results_datasets}
\end{table*}


==> tables/score_agg_with_program_judges.tex <==
%%%%%%% Previous version of table ---- Uncomment for shades of gray %%%%%%%
% \begin{table}[]
% \caption{Performance on different datasets using both LLM and program judges. MAE 
% %(lower is better) 
% and Kendall’s $\tau$ 
% %(higher is better) 
% are reported. Program judges are beneficial in FeedbackQA but may introduce noise in HelpSteer2 and UltraFeedback. In both cases, $\SYSNAME$ consistently outperforms other baselines.}\label{tab:results_program_judges}
% \centering
% \resizebox{0.6\textwidth}{!}{%
% \begin{tabular}{@{}c|cc|cc|cc@{}}
% \toprule
%  & \multicolumn{2}{c|}{\textbf{FeedbackQA}} & \multicolumn{2}{c|}{\textbf{HelpSteer2}} & \multicolumn{2}{c}{\textbf{UltraFeedback}} \\ \cmidrule(l){2-7} 
%  & \multicolumn{1}{c|}{MAE ($\downarrow$)} & $\tau$ ($\uparrow$) & \multicolumn{1}{c|}{MAE ($\downarrow$)} & $\tau$ ($\uparrow$) & \multicolumn{1}{c|}{MAE ($\downarrow$)} & $\tau$ ($\uparrow$) \\ \midrule
% \rowcolor[HTML]{EFEFEF} 
% MV & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.8607} & 0.3815 & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}1.0244} & \textbf{0.1465} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.8751} & 0.3179 \\
% AVG & \multicolumn{1}{c|}{0.8128} & 0.4671 & \multicolumn{1}{c|}{1.1012} & 0.1268 & \multicolumn{1}{c|}{1.0371} & \textbf{0.3733} \\
% \rowcolor[HTML]{EFEFEF} 
% UWS & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.8179} & \textbf{0.4816} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.9992} & 0.1040 & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.9534} & 0.3047 \\
% CARE & \multicolumn{1}{c|}{\textbf{0.7582}} & 0.4796 & \multicolumn{1}{c|}{\textbf{0.9800}} & 0.1398 & \multicolumn{1}{c|}{\textbf{0.7351}} & 0.3520 \\ \bottomrule
% \end{tabular}%
% }
% \end{table}


%%%%%%% Playing with colors, MAE is error - so reddish color %%%%%%%
% \begin{table}[]
% \caption{Performance on different datasets using both LLM and program judges. Program judges are beneficial in FeedbackQA but may introduce noise in HelpSteer2 and UltraFeedback. In both cases, $\SYSNAME$ consistently outperforms other baselines.}\label{tab:results_program_judges}
% \centering
% \resizebox{0.6\textwidth}{!}{%
% \begin{tabular}{@{}c|cc|cc|cc@{}}
% \toprule
 % & \multicolumn{2}{c|}{\textbf{FeedbackQA}} & \multicolumn{2}{c|}{\textbf{HelpSteer2}} & \multicolumn{2}{c}{\textbf{UltraFeedback}} \\ \cmidrule(l){2-7} 
 % & \multicolumn{1}{c|}{\cellcolor{red!30}MAE ($\downarrow$)} & \cellcolor{green!30}$\tau$ ($\uparrow$) & \multicolumn{1}{c|}{\cellcolor{red!30}MAE ($\downarrow$)} & \cellcolor{green!30}$\tau$ ($\uparrow$) & \multicolumn{1}{c|}{\cellcolor{red!30}MAE ($\downarrow$)} & \cellcolor{green!30}$\tau$ ($\uparrow$) \\ \midrule

% MV & \multicolumn{1}{c|}{\cellcolor{red!20}0.8607} & \cellcolor{green!20}0.3815 & \multicolumn{1}{c|}{\cellcolor{red!20}1.0244} & \textbf{\cellcolor{green!20}0.1465} & \multicolumn{1}{c|}{\cellcolor{red!20}0.8751} & \cellcolor{green!20}0.3179 \\
% AVG & \multicolumn{1}{c|}{\cellcolor{red!10}0.8128} & \cellcolor{green!10}0.4671 & \multicolumn{1}{c|}{\cellcolor{red!10}1.1012} & \cellcolor{green!10}0.1268 & \multicolumn{1}{c|}{\cellcolor{red!10}1.0371} & \textbf{\cellcolor{green!10}0.3733} \\ 
% UWS & \multicolumn{1}{c|}{\cellcolor{red!20}0.8179} & \textbf{\cellcolor{green!20}0.4816} & \multicolumn{1}{c|}{\cellcolor{red!20}0.9992} & \cellcolor{green!20}0.1040 & \multicolumn{1}{c|}{\cellcolor{red!20}0.9534} & \cellcolor{green!20}0.3047 \\
% CARE & \multicolumn{1}{c|}{\textbf{\cellcolor{red!10}0.7582}} & \cellcolor{green!10}0.4796 & \multicolumn{1}{c|}{\textbf{\cellcolor{red!10}0.9800}} & \cellcolor{green!10}0.1398 & \multicolumn{1}{c|}{\textbf{\cellcolor{red!10}0.7351}} & \cellcolor{green!10}0.3520 \\ \bottomrule
% \end{tabular}%
% }
% \vspace{-1mm}
% \end{table}


\begin{table*}[t!]
\caption{Performance on different datasets using both LLM and program judges. Program judges are beneficial in FeedbackQA but may introduce noise in HelpSteer2 and UltraFeedback. In both cases, $\SYSNAME$ consistently outperforms other baselines.}
\label{tab:results_program_judges}
\centering
\sisetup{
  round-mode=places,
  round-precision=4,
  table-format=1.4,
  table-number-alignment=center
}
\small
\begin{tabularx}{0.69\textwidth}{@{}l *{6}{S}@{}}
\toprule
 & \multicolumn{2}{c}{\textbf{FeedbackQA}} & \multicolumn{2}{c}{\textbf{HelpSteer2}} & \multicolumn{2}{c}{\textbf{UltraFeedback}} \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
 & {\cellcolor{blue!10}MAE ($\downarrow$)} & {\cellcolor{teal!10}$\tau$ ($\uparrow$)} & {\cellcolor{blue!10}MAE ($\downarrow$)} & {\cellcolor{teal!10}$\tau$ ($\uparrow$)} & {\cellcolor{blue!10}MAE ($\downarrow$)} & {\cellcolor{teal!10}$\tau$ ($\uparrow$)} \\ 
\midrule
MV   & {\cellcolor{blue!10}0.8607} & {\cellcolor{teal!10}0.3815} & {\cellcolor{blue!10}1.0244} & {\cellcolor{teal!10}\textbf{0.1465}} & {\cellcolor{blue!10}0.8751} & {\cellcolor{teal!10}0.3179} \\
AVG  & {\cellcolor{blue!10}0.8128} & {\cellcolor{teal!10}0.4671} & {\cellcolor{blue!10}1.1012} & {\cellcolor{teal!10}0.1268} & {\cellcolor{blue!10}1.0371} & {\cellcolor{teal!10}\textbf{0.3733}} \\
UWS  & {\cellcolor{blue!10}0.8179} & {\cellcolor{teal!10}\textbf{0.4816}} & {\cellcolor{blue!10}0.9992} & {\cellcolor{teal!10}0.1040} & {\cellcolor{blue!10}0.9534} & {\cellcolor{teal!10}0.3047} \\
CARE & {\cellcolor{blue!10}\textbf{0.7582}} & {\cellcolor{teal!10}0.4796} & {\cellcolor{blue!10}\textbf{0.9800}} & {\cellcolor{teal!10}0.1398} & {\cellcolor{blue!10}\textbf{0.7351}} & {\cellcolor{teal!10}0.3520} \\ 
\bottomrule
\end{tabularx}
\vspace{-5mm}
\end{table*}

==> tables/score_agg_with_program_judges_old.tex <==
\begin{table*}[t]
  \centering

  \begin{minipage}[t]{0.32\textwidth}
    \centering
    \caption*{\textbf{FeedbackQA}}
    \begin{tabular}{lrr}
      \toprule
       & MAE ($\downarrow$) & $\tau$ ($\uparrow$)\\
      \midrule
      MV   & 0.8607 & 0.3815 \\
      AVG  & 0.8128 & 0.4671 \\
      UWS  & 0.8178 & \textbf{0.4816} \\
      CARE & \textbf{0.7582} & 0.4796 \\
      \bottomrule
    \end{tabular}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.32\textwidth}
    \centering
    \caption*{\textbf{HelpSteer2}}
    \begin{tabular}{lrr}
      \toprule
      & MAE ($\downarrow$) & $\tau$ ($\uparrow$)\\
      \midrule
      MV   & 1.0244 & \textbf{0.1465} \\
      AVG  & 1.1012 & 0.1268 \\
      UWS  & 0.9992 & 0.1040 \\
      CARE & \textbf{0.9800} & 0.1398 \\
      \bottomrule
    \end{tabular}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.32\textwidth}
    \centering
    \caption*{\textbf{UltraFeedback}}
    \begin{tabular}{lrr}
      \toprule
      & MAE ($\downarrow$) & $\tau$ ($\uparrow$)\\
      \midrule
      MV   & 0.8751 & 0.3179 \\
      AVG  & 1.0371 & \textbf{0.3733} \\
      UWS  & 0.9534 & 0.3047 \\
      CARE & \textbf{0.7351} & 0.3520 \\
      \bottomrule
    \end{tabular}
  \end{minipage}
  \caption{Performance on different datasets using both LLM and program judges. MAE (lower is better) and Kendall’s $\tau$ (higher is better) are reported. Program judges are beneficial in FeedbackQA but may introduce noise in HelpSteer2 and UltraFeedback. In both cases, $\SYSNAME$ consistently outperforms other baselines.}
  \label{tab:results_program_judges}
\end{table*}

